Evidence for B+ -> K*0bar K*+

We present measurements of the branching fraction and fraction of longitudinal polarization for the decay B+ -> K*0bar K*+ with a sample of 467 +/- 5 million BBbar pairs collected with the BaBar detector at the PEP-II asymmetric-energy e+e- collider at the SLAC National Accelerator Laboratory. We obtain the branching fraction Br(B+ -> K*0bar K*+) = (1.2 +/- 0.5 +/- 0.1) x 10^{-6} with a significance of 3.7 standard deviations including systematic uncertainties. We measure the fraction of longitudinal polarization f_L = 0.75+0.16-0.26 +/- 0.03. The first error quoted is statistical and the second is systematic.

==> abstract.tex <==
%\documentclass[aps,prl]{revtex4}
%\begin{document}
We present measurements of the branching fraction and longitudinal
polarization for the decay $B^+ \rightarrow \overline{K}^{*0} K^{*+}$
with a sample of $467\pm5$ million $B\overline{B}$ pairs collected
with the BaBar detector at the PEP-II asymmetric-energy $e^+e^-$
collider at the SLAC National Accelerator Laboratory.  We obtain the
branching fraction ${\cal B} (B^+ \rightarrow \overline{K}^{*0}
K^{*+}) = (1.2 \pm 0.5 \pm 0.1)\times 10^{-6}$ with a significance of
3.7 standard deviations including systematic uncertainties.  We
measure the fraction of longitudinal polarization $f_{L} =
0.75^{+0.16}_{-0.26}\pm0.03$. The first error quoted is statistical
and the second is systematic.

%\end{document}

